Quality-Aware Personalized AI Service Provisioning in UAV-Assisted 6G Networks

In sixth-generation (6G) artificial intelligence (AI) services, two quality dimensions should be jointly addressed: conventional quality (e.g., latency) and Quality of AI Services (QoAIS; output fidelity, continuity, personalization). Existing methods emphasize conventional quality, while neglecting QoAIS, particularly for personalized outputs in dynamic aerial-terrestrial settings. This paper introduces HyPE, a Hybrid Predictive-in-context-lEarning framework for holistically quality-aware personalized AI service provisioning in Unmanned Aerial Vehicle (UAV)-assisted 6G networks. HyPE integrates: (i) mobility-aware prediction to forecast spatio-temporal request distributions, (ii) learning-augmented decision leveraging Large Language Model (LLM)-based reasoning to optimize UAV trajectories and inference assignments, and (iii) pre-/post-processing service placement and routing using heuristics. We formulate an optimization problem for joint trajectory planning, service placement, and routing, and present HyPE as a scalable alternative to intractable optimal solutions. Simulations with empirical mobility traces and heterogeneous AI workloads show near-optimal coverage, reduced end-to-end latency, sustained QoAIS-driven, and continuity-based service personalization versus optimization and state-of-the-art baselines. The results highlight the promise of predictive learning-augmented provisioning for elastic, user-centric AI in 6G.

==> Tables/tab1.tex <==
\renewcommand{\arraystretch}{1.45}
\begin{table}[t!]
\centering
\caption{List of notations used in the problem formulation.}
\vspace{-5pt}
\label{table:notations}
\begin{tabular}{|c|l|}
\hline
\textbf{Notation}              & \textbf{Description}                                                             \\ \hline
$\mathcal{G}(\mathcal{N}, \mathcal{L}, \mathcal{P})_t$ & Aerial-terrestrial edge-cloud network graph at time $t$ \\ \hline

$\boldsymbol{\mathcal{N}} / \boldsymbol{\mathcal{A}}$     & Set of network nodes / predefined areas \\ \hline
$\boldsymbol{\mathcal{U}} / \boldsymbol{\mathcal{R}} $      & Set of (active UEs / Requests)    \\ \hline
$\boldsymbol{\mathcal{L}}_t / \boldsymbol{\mathcal{P}}_t $ & Set of (wireless links / active paths) at time $t$ \\ \hline

$t \in \boldsymbol{\mathcal{T}}$  & Time frame (of Total service time)                                            \\ \hline
$\mathcal{F}^{pr}_f \in \boldsymbol{\mathcal{F}}^{pr}_s$    & function $f$ (of pre-processing functions set) \\ \hline
% $\mathcal{F}^{in}_f \in \boldsymbol{\mathcal{F}}^{in}_s$    & function $f$ (of inference functions set) \\ \hline
$\mathcal{F}^{po}_f \in \boldsymbol{\mathcal{F}}^{po}_s$    & function $f$ (of post-processing functions set) \\ \hline 
\hline



$u_{r} / \mathcal{S}_r$ & (UE who send / AI service) of request $r$  \\ \hline
$\mathcal{T}^{en}_r$  & Entry time of UE request $r$    \\ \hline
$\Delta_r$    & Time window that the request $r$ should be processed                          \\ \hline
$\mathcal{I}_{u,a,t}$         & Indicator for UE $u$ located in area $a$ at time $t$   \\ \hline 

$\widecheck{\mathcal{L}}_{r}$ & Network bandwidth required for request $r$ \\ \hline
% $\widecheck{\mathcal{B}}_{r,t}$ & Traffic burstiness of request $r$ \\ \hline
$\widecheck{\mathcal{Z}}_{r,t}$ & Maximum packet size of request $r$ \\ \hline
$\widecheck{\mathcal{C}}^{pr}_{r,f}$ & Min pre-process capacity required for function $f$ of $r$ \\ \hline
$\widecheck{\mathcal{C}}^{in}_{r}$ & Min inference capacity required for request $r$ \\ \hline
$\widecheck{\mathcal{C}}^{po}_{r,f}$ & Min post-process capacity required for function $f$ of $r$ \\ \hline

$\widecheck{\mathcal{Q}}^{ou}_{r}$    & Output Quality requirement for request $r$        \\ \hline
% $\widecheck{\mathcal{Q}}^{pe}_{u}$    & Personalized response requirement for user $u$ \\ \hline
$\widecheck{\mathcal{Q}}^{la}_{r}$    & Latency requirement for request $r$       \\ \hline
\hline

$\pi^{pr}_{s}$    & Number of pre-process functions of service $s$       \\ \hline
$\pi^{po}_{s}$    & Number of post-process functions of service $s$       \\ \hline
$\mathcal{T}^{du}_s$ & Total time for delivering service $s$ \\ \hline
\hline



% $\widehat{\mathcal{C}}^{qu}_n $      & Inference capacity of node $n$ \\ \hline
$\widehat{\mathcal{C}}^{ca}_n$      & Computing capacity of node $n$ \\ \hline
$\overline{Q}_n$ & Output quality of node $n$ \\ \hline % (based on its capacity to use distilled or full model) 
$\widehat{\mathcal{L}}_l$      & Bandwidth capacity of link $l$ \\ \hline
$\mathcal{H}_{p,t} / \mathcal{T}_{p,t}$ & Head/Tail node of path $p$ at time frame $t$  \\ \hline
$\mathcal{J}_{p,l,t}$          & The inclusion of link $l$ in path $p$ at time frame $t$ \\ \hline
% $\mathcal{D}_{r,l,t}$ & Latency experienced by request $r$ over link $l$ at time $t$   \\ \hline
$\mathcal{A}_{a,a'}$ & if area $a$ and $a'$ are adjacent   \\ \hline
\hline







$\mathcal{X}^{pr}_{r,t}$ & if pre-process function $f$ of $r$ is selected at $t$ \\ \hline
$\mathcal{X}^{in}_{r,t}$ & if Inference function $f$ of $r$ is selected at $t$ \\ \hline
$\mathcal{X}^{po}_{r,t}$ & if post-process function $f$ of $r$ is selected at $t$ \\ \hline

% $\mathcal{Y}^{pr}_{f,n,t}$ & if pre-process function $f$ is placed on node $n$ at time frame $t$ \\ \hline
$\mathcal{Y}_{f,n,t}$ & if function $f$ is placed on node $n$ at time frame $t$ \\ \hline
$\mathcal{Y}^{in}_{r,n,t}$ & if request $r$ is reasoned node $n$ at time frame $t$ \\ \hline
% $\mathcal{Y}^{po}_{f,n,t}$ & if post-process function $f$ is placed on node $n$ at time frame $t$ \\ \hline

$\mathcal{S}_{n,a,t}$ & if node $n$ is deployed in area $a$ at time frame $t$ \\ \hline
$\mathcal{B}_{u,n,t}$ & if UE $u$ is connected to node $n$ at time frame $t$ \\ \hline
% $\mathcal{R}^{pr}_{r,p,t}$ & if path $p$ is selected for pre-processing of request $r$ at time frame $t$ \\ \hline
$\mathcal{R}_{r,p,t}$ & if path $p$ is selected for request $r$ at time frame $t$ \\ \hline
% $\mathcal{R}^{po}_{r,p,t}$ & if path $p$ is selected for post-processing of request $r$ at time frame $t$ \\ \hline
$\mathcal{L}_{n,n',t}$ & if there is a link between $n$ and $n'$ at time $t$  \\ \hline
% $\overrightarrow{\mathcal{R}}_{r,p,t}$ & if path $p$ is selected for request $r$ at time frame $t$ \\ \hline
\end{tabular}
\vspace{-2pt}
\end{table}
